Zemi: Learning Zero-Shot Semi-Parametric Language Models from Multiple Tasks

Although large language models have achieved impressive zero-shot ability, the huge model size generally incurs high cost. Recently, semi-parametric language models, which augment a smaller language model with an external retriever, have demonstrated promising language modeling capabilities. However, it remains unclear whether such semi-parametric language models can perform competitively well as their fully-parametric counterparts on zero-shot generalization to downstream tasks. In this work, we introduce $\text{Zemi}$, a zero-shot semi-parametric language model. To our best knowledge, this is the first semi-parametric language model that can demonstrate strong zero-shot performance on a wide range of held-out unseen tasks. We train $\text{Zemi}$ with a novel semi-parametric multitask prompted training paradigm, which shows significant improvement compared with the parametric multitask training as proposed by T0. Specifically, we augment the multitask training and zero-shot evaluation with retrieval from a large-scale task-agnostic unlabeled corpus. In order to incorporate multiple potentially noisy retrieved augmentations, we further propose a novel $\text{augmentation fusion}$ module leveraging perceiver resampler and gated cross-attention. Notably, our proposed $\text{Zemi}_\text{LARGE}$ outperforms T0-3B by 16% on all seven evaluation tasks while being 3.9x smaller in model size.

==> sections/2_related_work.tex <==
\section{Related Work}


\subsection{Semi-parametric models}

Traditionally, semi-parametric models have been widely applied to specific knowledge-intensive NLP tasks such as open-domain question answering~\citep{DrQA,ORQA,REALM,multi_passage_bert,DPR,BERTserini,RAG,FiD}. 
One representative paradigm is the retriever-reader framework where the retriever first retrieves top k (e.g., 100) relevant passages from a large corpus, and then the reader either generates or extracts the answer conditioned on the query and the retrieved passages. 
% For example, RAG~\citep{RAG} trains an end-to-end model with a parametric seq2seq transformer and a non-parametric dense retriever. 
% Building upon RAG, 
% FiD~\citep{FiD} combines the encoded query and documents before feeding them into a decoder, making it possible for the decoder to consider multiple document representations at the same time.
One limitation of those traditional retriever-reader models is that they are designed to solve specific tasks, for example, retrieving from Wikipedia for answering trivia questions~\citep{joshi2017triviaqa}.
In this work, we retrieve from a large-scale \textbf{task-agnostic} corpus, C4~\citep{t5}, which is the unlabeled pre-training corpus of our backbone model.

Recent advancements in semi-parametric language models~\citep{knn-lm, spalm, retro, memory_aug_lm} focus on improving language modeling with a relatively small language model and a retrieval system based on a large-scale corpus. \cite{knn-lm} and \cite{spalm} share the idea of extending a pretrained language model by linearly interpolating it with a k-nearest neighbor model. \cite{retro} proposed to improve language model pretraining with a retrieval-enhanced transformer with chunked cross-attention layers.
% , which has chunked cross-attention layer interleaved with the original attention layers in the decoder. 
% \cite{memory_aug_lm} proposed training language models with memory augmentation. 
Although the aforementioned semi-parametric language models have shown competitive performance on language modeling compared with fully-parametric counterparts such as GPT-3~\citep{gpt3}, they are rarely evaluated on unseen downstream tasks, leaving it unexplored whether semi-parametric language models can perform competitively well on zero-shot task generalization. While concurrent work~\citep{meta_atlas} showed initial success in few-shot settings relying on Fusion-in-Decoder (FiD)~\citep{FiD} framework, this work focus on the more challenging \textbf{zero-shot} settings. Furthermore, instead of reusing FiD framework as in \cite{meta_atlas}, we show that our newly proposed semi-parametric architecture is more effective than FiD due to the \textbf{gated mechanism}.

% \subsection{Open-Domain Question Answering}
% Current Open-Domain Question Answering approaches often adopt a retriever-reader framework \citep{DrQA,BERTserini,REALM,DPR,RAG,FiD}, where the retriever first retrieves top k (i.e., 100) relevant passages from a large corpus and then the reader either generate or extract the answer conditioned on the retrieved passages. One limitation of the retriever-reader models is that they often require task-specific pre-training or fine-tuning which requires large amount of human annotated data. Recent advancement in large-scale generative language models \citep{gpt2,gpt3,t5,t0,internet-augmented-lm} provide a series of alternative retriever-free methods where we treat the language model itself as a knowledge base and directly generate the answer to each question. However, recent research \citep{wei2022emergent, gpt3} shows that such ability often requires the model size to be larger than a certain threshold, i.e., 10B, which is out of reach for most researchers. One promising line of work for reducing the model size while attaining the strong reasoning ability is to use semi-parametric models, where we augment a smaller language model with retrieval on a external knowledge base. One may notice that the idea of semi-parametric model is very similar to the retriever-reader model in open-domain question answering literature. However, at the time writing this paper, most previous work on semi-parametric model only focuses on language modeling and rarely evaluated on unseen downstream tasks without task-specific fine-tuning. 

\subsection{Massive multitask prompted training}
Based on the assumption that the reasonable zero-shot ability of large language models may come from implicit multitask learning during pretraining, recent studies~\citep{t0, FLAN, CrossFit, benchmarking1600} have demonstrated that explicitly training a language model on a mixture of diverse tasks can effectively improve its zero-shot performance on unseen tasks. For example, a multitask fine-tuned 11B T0 model~\citep{t0} can outperform the 175B GPT-3 on a variety of held-out unseen tasks.
Followup work~\citep{what_lm_arch_for_zero_shot_generalization} shows that encoder-decoder model architecture is particularly suitable for multitask finetuning. 
In this work, we extend T0's multitask prompted training to \textbf{semi-parametric multitask prompted training}, where we further augment the training and evaluation instances with retrieved documents. Notably, our work is distinguished from previous work ReCross~\citep{Lin2022UnsupervisedCG}, which uses upstream training data for augmentation, in twofold. First, we retrieve documents from a much larger task-agnostic corpus instead of clean upstream training instances. Second, in addition to directly concatenating the augmentation with the input just as FiD~\citep{FiD}, we further propose a novel augmentation fusion module to handle a larger number of potentially noisy retrieved augmentations.


\subsection{Fusion of retrieved augmentations}
\label{sec:related_work_fusion_of_augmentation}
In this work, the main challenge in designing the semi-parametric language model architecture is to attain the ability to handle multiple potentially noisy retrieved documents.
Existing methods on incorporating external texts fall in two categories, \textit{concatenation based}~\citep{Lin2022UnsupervisedCG, gpt3, generated_knowledge_prompt, RAG, wang2022training} and \textit{cross-attention based}~\citep{FiD, DoHA, retro}. Concatenation-based methods directly concatenate the retrieved texts with the input and use a unified self-attention to incorporate the augmentations. 
This method is highly expressive but the number of texts that can be added is strictly limited to the model's maximum input length. Cross-attention-based methods can take into account a larger number of texts, but they still lack an explicit design for preventing the model from paying attention to the noisy ones. Inspired by recent visual language models~\cite{flamingo,yu2022coca,li2022blip,jiang2022vima}, we propose to leverage perceiver resamplers~\citep{perceiver_IO} and gated cross-attention layers for incorporating external texts. Although originally proposed for vision-language fusion in Flamingo~\citep{flamingo}, we find that the idea can be effectively transferred to do augmentation fusion with potentially noisy retrieved documents.
Furthermore, we identify two key differences from Flamingo: first, we use a much smaller encoder-decoder model that is jointly trained with the newly initialized layers instead of frozen layers. Second, instead of inserting the gated cross-attention module into a large frozen language model~\citep{chinchilla}, we add only one layer of gated cross-attention on top of the encoder to alleviate the need for extensive pre-training.


==> sections/additional_analysis.tex <==

% \subsection{Why semi-parametric multitask training works?}
% \label{sec:additional_ablation}

\begin{wrapfigure}{r}{7cm}
\vspace{-10pt}
% \begin{figure}[thb]
\begin{minipage}{0.51\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/shuffle_strategy.png}
    \vspace{-15pt}
    \caption{Augmentation shuffling strategies.}
    % Detailed results on each task can be found in Table~\ref{table:aug_shuffle_single_task},\ref{table:aug_shuffle_multitask}. }
    \label{fig:shuffle_strategy}
\end{minipage}
\vspace{-5pt}
\end{wrapfigure}

In Table~\ref{table:main_result}, we show that existing augmentation fusion methods cannot achieve visible positive gain due to the noisy retrieval as visualized in Appendix~\ref{sec:retrieval_examples}. In contrast, \ours{} is able to achieve significant improvement by leveraging the noisy retrieved augmentations. In this section, we aim to further investigate \textit{what is the key benefit of the retrieval augmentation that helps improve zero-shot task generalization}.
% In this section we aim to investigate why \textit{semi-parametric multitask training} helps further improve zero-shot task generalization compared with \textit{parametric multitask training}. The main goal is to explore what kind of additional information derived from the retrieval that is of most importance towards effective zero-shot generalization. 
To this end, we design an additional ablation study on the retrieval augmentation. We introduce two types of perturbations on the original retrieved augmentations, i.e., \textbf{in-task shuffle} and \textbf{cross-task shuffle}. As illustrated in Figure~\ref{fig:shuffle_strategy}, for in-task Shuffle, during both training and evaluation, we replace the augmentation of each instance with a randomly picked retrieved augmentation from another instance \textbf{within the same task}. For cross-task shuffle, we replace the augmentation of each instance with a randomly picked retrieved augmentation from \textbf{a different task} in the entire training and evaluation mixtures. 
Table~\ref{table:aug_shuffle_multitask} shows the averaged relative gain against the \textit{No Aug} baseline.

\input{tables/aug_shuffle_multitask}

% \begin{wrapfigure}{r}{7cm}
% \vspace{-15pt}
% % \begin{figure}[thb]
% \begin{minipage}{0.5\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/multi_task_and_single_task_avg_delta_mean_no_hatch.pdf}
%     \vspace{-20pt}
%     \caption{Impact of changing augmentations. The scores are the averaged relative gain on the mean accuracy across seven tasks against the \textit{No Aug} baseline as shown in Table~\ref{table:main_result}. \zhenhailong{report multitask only; report only in-task shuffle and x-task shuffle;}}
%     % Detailed results on each task can be found in Table~\ref{table:aug_shuffle_single_task},\ref{table:aug_shuffle_multitask}. }
%     \label{fig:aug_shuffle_analysis}
% \end{minipage}
% % \end{figure}
% \vspace{-10pt}
% \end{wrapfigure}

% \noindent \textbf{It is the overall semi-parametric training paradigm rather than the specific content of the retrieved augmentations that helps improve zero-shot task generalization.} Comparing the left four bars in Figure~\ref{fig:aug_shuffle_analysis}, i.e., using original augmentations v.s. using N/A augmentations during inference, we find that for both single-task and multi-task setting, the zero-shot performance does not decrease and even increases with dummy augmentations. This is showing that, during inference, the learned model gated out almost all information from the augmentation and focus only on the prompted input. Thus, the significant positive gain against \textit{No Aug} demonstrates that it is the overall semi-parametric training paradigm that helps the model learn generalizable abilities for solving unseen tasks. Then a natural question is, if the specific content of the retrieved augmentation is not the key towards the benefits, what would be?

 Our main observation is that \textbf{capturing task-level correlation} is the key factor towards effective retrieval augmentation. First, we observe that doing in-task or cross-task shuffle can hurt the performance, which is intuitive since the shuffling weakens the instance-level correlation between the input and the augmentations. However, interestingly, we find that cross-task shuffle has a smaller negative impact on the performance than the in-task shuffle. This is showing that capturing the overall task-level correlation between the input instances and the augmentations is more important than capturing instance-level correlation. Thus, from a data augmentation perspective, we hypothesis that augmenting multitask training with retrieved documents from a large-scale task-agnostic corpus, despite being noisy, can encourage the model to learn generalizable abilities for solving various kinds of tasks instead of one specific task.

% capturing the general information of the current 
% while in the multi-task setting the observation reversed. This is showing that if the optimization objective is a single task, the key requirement of the augmentations is to capture the general \textbf{task-level features of the current task}. Intuitively, if our optimization objective is a wide range of tasks, the key to effective augmentation becomes capturing the \textbf{overall task-level features of multiple tasks}.

==> tables/aug_shuffle_multitask.tex <==

% \begin{table*}[!hbt]
\begin{wraptable}{r}{7cm}
\vspace{-10pt}
\small
\centering
\setlength\tabcolsep{3pt}
% \setlength\extrarowheight{1pt}
% \begin{tabularx}{\linewidth}{l|CCCC}
\begin{tabular}{c | c || c | c | c }
\toprule

\multirow{2}{*}{\textbf{Task}} &
\multirow{2}{*}{\textbf{No Aug}}&
\multirow{1}{*}{\textbf{\ours{}}}&
\multirow{1}{*}{\textbf{In-task}}&
\multirow{1}{*}{\textbf{Cross-task}}
\\
& & \textbf{Original} & \textbf{Shuffle} & \textbf{Shuffle}
\\
\midrule
OBQA    & \;36.64  &  35.55  & \,36.02  & \,34.49 \\
Piqa    & \;60.24  &  59.23  & \,60.00  & \,59.30 \\
RT      & \;64.11           &  68.58   & \,63.04   & \,71.97\\
CB      & \;41.46           &  50.05    & \,47.92 & \,42.08\\
COPA    & \;68.46           &  63.57   & \,64.94   & \,70.41  \\
WiC     & \;49.92           &  49.56  & \,50.47  & \,52.40 \\
HSwag   & \;27.97           &  29.68   & \,29.09 & \,29.49 \\

\midrule
Rel $\Delta$ Avg    & \;0.00   & +3.04   & \,+1.77  & \,+2.80 \\
% Median $\Delta$ & 0.00 & 0.00 & +1.70 & +0.47 & +1.65 & +0.47 & +1.43 & +0.78 & +1.69 & +0.55\\
\bottomrule
% \end{tabularx}
\end{tabular}

\caption{Impact of perturbing augmentations on semi-parametric multitask prompted training to zero-shot task generalization.}
\label{table:aug_shuffle_multitask}
\end{wraptable}
% \end{table*}









% \begin{table*}[!hbt]
% \small
% \centering
% \setlength\tabcolsep{3pt}
% % \setlength\extrarowheight{1pt}
% % \begin{tabularx}{\linewidth}{l|CCCC}
% \begin{tabular}{c | cc || cc | cc | cc | cc }
% \toprule

% \multirow{2}{*}{\textbf{Task}} &
% \multicolumn{2}{c||}{\textbf{No Aug}}&
% \multicolumn{2}{c|}{\textbf{Semi-T0 (Original)}}&
% \multicolumn{2}{c|}{\textbf{N/A Aug @Eval}} &
% \multicolumn{2}{c|}{\textbf{In-task Shuffle}} &
% \multicolumn{2}{c}{\textbf{X-task Shuffle}}
% \\
% &
% \;Mean & Median &
% \quad Mean & Median &
% \,Mean & Median &
% \,Mean & Median &
% \,Mean & Median
% \\
% \midrule
% OBQA    & \;\textbf{36.64} & \textbf{36.52}           & \quad 35.55 & 35.16  & \,35.55 & 35.16  & \,36.02 & 36.13  & \,34.49 & 33.40\\
% Piqa    & \;\textbf{60.24} & \textbf{61.26}           & \quad 59.23 & 60.57  & \,59.24 & 60.82  & \,60.00 & 61.05  & \,59.30 & 60.40\\
% RT      & \;64.11 & 64.11           & \quad 68.58 & 68.58  & \,\textbf{69.68} & \textbf{69.68}  & \,63.04 & 63.42  & \,71.97 & 71.97\\
% CB      & \;41.46 & 50.00           & \quad \textbf{50.05} & \textbf{58.59}  & \,49.90 & 57.81  & \,47.92 & 56.25  & \,42.08 & 48.44\\
% COPA    & \;68.46 & 69.92           & \quad 63.57 & 63.67  & \,65.29 & 65.18  & \,64.94 & 66.02  & \,\textbf{70.41} & \textbf{71.48} \\
% WiC     & \;49.92 & 50.08           & \quad 49.56 & 49.77  & \,49.56 & 49.77  & \,50.47 & 50.00  & \,\textbf{52.40} & \textbf{52.19}\\
% HSwag   & \;27.97 & 27.91           & \quad \textbf{29.68} & \textbf{29.39}  & \,29.63 & 29.32  & \,29.09 & 29.10  & \,29.49 & 29.35\\

% \midrule
% Avg             & \;49.83 & 51.40   & \quad 50.89 & 52.25  & \,51.26 & \,52.53 & \,50.27 & 51.71 & \,\textbf{51.45} & \textbf{52.46}\\
% Rel $\Delta$ Avg    & \;0.00 & 0.00     & \quad +3.04 & +2.15  & \,\textbf{+3.57} & \textbf{+2.50}   & \,+1.77 & +1.22 & \,+2.80 & +1.54\\
% % Median $\Delta$ & 0.00 & 0.00 & +1.70 & +0.47 & +1.65 & +0.47 & +1.43 & +0.78 & +1.69 & +0.55\\
% \bottomrule
% % \end{tabularx}
% \end{tabular}
% \caption{Impact of changing augmentation on semi-parametric multitask prompted training to zero-shot task generalization. X-task Shuffle is short for Cross-task Shuffle. \zhenhailong{remove N/A, remove median}}
% \label{table:aug_shuffle_multitask}
% \end{table*}



==> tables/scale_to_large.tex <==
\begin{wraptable}{r}{7cm}
\vspace{-10pt}
\begin{minipage}{0.5\textwidth}
\small
\centering
\setlength\tabcolsep{3pt}
% \setlength\extrarowheight{1pt}
% \begin{tabularx}{\linewidth}{l|CCCC}
    \begin{tabular}{c | cc || cc }
    \toprule
    
    \multirow{2}{*}{\textbf{Task}} &
    \multicolumn{2}{c||}{\textbf{No Aug large}}&
    \multicolumn{2}{c}{\textbf{\ours{} large (Ours)}}
    \\
    &
    \;Mean & Median &
    Mean$^{\Delta}$ & Median$^{\Delta}$
    \\
    \midrule
    OBQA        & \;50.50 & 50.78 & \textbf{51.49$^{+1.95}$} & \textbf{52.60$^{+3.58}$} \\
    Piqa        & \;65.50 & 67.34 & \textbf{67.85$^{+3.58}$} & \textbf{67.45$^{+0.16}$} \\
    RT          & \;82.23 & 82.23 & \textbf{84.13$^{+2.31}$} & \textbf{84.13$^{+2.31}$} \\
    CB          & \;52.40 & 57.81 & \textbf{62.14$^{+18.60}$} & \textbf{69.64$^{+20.46}$} \\
    COPA        & \;80.02 & 82.14 & \textbf{84.50$^{+5.60}$} & \textbf{86.00$^{+4.70}$} \\
    WiC         & \;50.16 & \textbf{50.00} & \textbf{50.44$^{+0.57}$} & 49.92$^{-0.16}$ \\
    HSwag       & \;34.12 & 33.92 & \textbf{35.79$^{+4.90}$} & \textbf{34.27$^{+1.04}$} \\
    
    \midrule
    Avg             & \;59.28 & 60.60 & \textbf{62.33} & \textbf{63.43} \\
    Avg $\Delta$    & \;0.00 & 0.00 & \textbf{+5.36} & \textbf{+4.58} \\
    \bottomrule
    % \end{tabularx}
    \end{tabular}
    \caption{\ours{} with T5-large backbone. }
    \label{table:scale_to_large}
\end{minipage}
\vspace{-10pt}
\end{wraptable}


% \begin{table*}[!hbt]
% \begin{minipage}{0.51\textwidth}
% We are interested in verifying if the benefit from semi-parametric multitask training can be scaled to larger models. To this end, we propose a larger variant of \ours{} budded as \textbf{\ours{} large}, where we replace the T5-base ($220$M) backbone with T5-large ($770$M). Correspondingly, we train a \textbf{No Aug large} baseline with T5-large as backbone. We keep the training mixture intact as \ours{} base. As shown in Table~\ref{sec:scale_to_large}, we observe an overall positive gain of \textbf{2.58\%} in mean which is even larger than the base version of \ours{}. This result shows the potential of building even larger variant of \ours{} models that can achieve even better performance. In the next section, we show the comparison to current state-of-the-art methods.
% \end{minipage}%
% \hspace{2pt}
% \begin{minipage}{0.48\textwidth}
% \small
% \centering
% \setlength\tabcolsep{3pt}
% % \setlength\extrarowheight{1pt}
% % \begin{tabularx}{\linewidth}{l|CCCC}
%     \begin{tabular}{c | cc || cc }
%     \toprule
    
%     \multirow{2}{*}{\textbf{Task}} &
%     \multicolumn{2}{c||}{\textbf{No Aug large}}&
%     \multicolumn{2}{c}{\textbf{\ours{} large (Ours)}}
%     \\
%     &
%     \;Mean & Median &
%     Mean$^{\Delta}$ & Median$^{\Delta}$
%     \\
%     \midrule
%     OBQA        & \;50.50 & 50.78 & \textbf{51.49}$^{+1.95}$ & \textbf{52.60}$^{+3.58}$ \\
%     Piqa        & \;65.50 & 67.34 & \textbf{66.95}$^{+2.21}$ & \textbf{69.18}$^{+2.74}$ \\
%     RT          & \;\textbf{84.98} & \textbf{84.98} & 84.13$^{-1.00}$ & 84.13$^{-1.00}$ \\
%     CB          & \;55.42 & 68.75 & \textbf{62.14}$^{+12.14}$ & \textbf{69.14}$^{+1.30}$ \\
%     COPA        & \;82.48 & 83.93 & \textbf{84.50}$^{+2.45}$ & \textbf{86.00}$^{+2.47}$ \\
%     WiC         & \;51.04 & \textbf{50.31} & \textbf{51.48}$^{+0.87}$ & 51.02$^{+1.40}$ \\
%     HSwag       & \;\textbf{36.00} & \textbf{35.48} & 35.79$^{-0.58}$ & 34.27$^{-3.40}$ \\
    
%     \midrule
%     Avg $\Delta$    & \;0.00 & 0.00 & \textbf{+2.58} & \textbf{+1.01} \\
%     % Median $\Delta$ & 0.00 & 0.00 & \textbf{+1.95} & \textbf{+1.40} \\
%     \bottomrule
%     % \end{tabularx}
%     \end{tabular}
%     \caption{Scale to T5-large backbone.}
%     \label{table:scale_to_large}

% \end{minipage}
% \end{table*}


